Generative Time Series Forecasting with Diffusion, Denoise, and Disentanglement

Time series forecasting has been a widely explored task of great importance in many applications. However, it is common that real-world time series data are recorded in a short time period, which results in a big gap between the deep model and the limited and noisy time series. In this work, we propose to address the time series forecasting problem with generative modeling and propose a bidirectional variational auto-encoder (BVAE) equipped with diffusion, denoise, and disentanglement, namely D3VAE. Specifically, a coupled diffusion probabilistic model is proposed to augment the time series data without increasing the aleatoric uncertainty and implement a more tractable inference process with BVAE. To ensure the generated series move toward the true target, we further propose to adapt and integrate the multiscale denoising score matching into the diffusion process for time series forecasting. In addition, to enhance the interpretability and stability of the prediction, we treat the latent variable in a multivariate manner and disentangle them on top of minimizing total correlation. Extensive experiments on synthetic and real-world data show that D3VAE outperforms competitive algorithms with remarkable margins. Our implementation is available at https://github.com/PaddlePaddle/PaddleSpatial/tree/main/research/D3VAE.

==> sec/10.checklist.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
%The checklist follows the references.  Please read the checklist guidelines carefully for information on how to answer these questions.  For each question, change the default \answerTODO{} to \answerYes{}, \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf justification to your answer}, either by referencing the appropriate section of your paper or providing a brief inline description.  For example: \begin{itemize} \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{experiment}.} \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.} \item Did you include the license to the code and datasets? \answerNA{} \end{itemize} Please do not modify the questions and only use the provided macros for your answers.  Note that the Checklist section does not count towards the page limit.  In your paper, please delete this instructions block and only keep the Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
   % \answerTODO{}
   \answerYes{}
  \item Did you describe the limitations of your work?
   % \answerTODO{}
   \answerYes{See~\cref{discuss} for details.}
  \item Did you discuss any potential negative societal impacts of your work?
    %\answerTODO{}
    \answerYes{We discuss the potential negative societal impacts in~\cref{discuss}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    %\answerTODO{}
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    %\answerTODO{}
    \answerYes{Our problem formulation and theoretical proof are described in~\cref{sec:method}, and all the theoretical results are with reasonable and necessary assumptions.}
  \item Did you include complete proofs of all theoretical results?
    %\answerTODO{}
    \answerYes{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    %\answerTODO{}
    \answerYes{We use six real-world datasets, for each of them is provided by URL or citation in~\cref{setting}.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    %\answerTODO{}
    \answerYes{See Section~\ref{experiment} and Appendix~\ref{exp}}
    \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
   % \answerTODO{}
   \answerYes{All the experimental results are repeated five times, the mean and standard deviation of the results are provided in~\cref{experiment}}
    \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Section~\ref{setting}}
    %\answerTODO{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    %\answerTODO{}
    \answerYes{The datasets and baseline models that used in this paper are all cited in~\cref{setting}.}
  \item Did you mention the license of the assets?
    %\answerTODO{}
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    %\answerTODO{}
    \answerYes{
    The newly introduced Wind dataset is publicly available at \url{https://github.com/PaddlePaddle/PaddleSpatial/tree/main/paddlespatial/datasets/WindPower}.
    }
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    %\answerTODO{}
    \answerYes{The datasets used in this paper are all public datasets, and we didn't use/curate data from other people.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    %\answerTODO{}
    \answerYes{The data we use doesn't contain any identifiable information or offensive content.}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    %\answerTODO{}
   \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
   % \answerTODO{}
   \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    %\answerTODO{}
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



